Covariant Spectator Theory of $np$ scattering: Deuteron form factors

The deuteron form factors are calculated using two model wave functions obtained from the 2007 CST high precision fits to $np$ scattering data. Included in the calculation are a new class of isoscalar $np$ interaction currents which are automatically generated by the nuclear force model used in these fits. If the nuclear model WJC2 is used, a precision fit ($\chi^2$/datum $\eqsim1$) to the Sick Global Analysis (GA) of all $ed$ elastic scattering data can be obtained by adjusting the unknown off-shell nucleon form factors $F_3(Q^2)$ (discussed before) and $F_4(Q^2)$ (introduced in this paper), and predicting the high $Q^2$ behavior of the neutron charge form factor $G_{En}(Q^2)$ well beyond the region where it has been measured directly. Relativistic corrections, isoscalar interaction currents, and off-shell effects are defined, discussed, and their size displayed. A rationale for extending $ed$ elastic scattering measurements to higher $Q^2$ is presented.

==> Body.tex <==
 0.001 &  1.003D+00 & -2.611D-07 & -3.334D-03 &  5.429D-10\;\; &  1.924D+00 &  1.793D+00 &  4.994D-03 & -2.247D-04\;\; &  2.548D+01 & -4.196D-01 & -2.725D-04 & -1.861D-04\;\;\cr
 0.101 &  8.576D-01 & -2.251D-03 & -3.308D-03 &  5.494D-06\;\; &  1.654D+00 &  1.527D+00 &  4.969D-03 & -2.402D-04\;\; &  2.189D+01 & -4.555D-01 & -1.918D-04 & -1.809D-04\;\;\cr
 0.201 &  5.988D-01 & -6.042D-03 & -3.232D-03 &  2.091D-05\;\; &  1.181D+00 &  1.064D+00 &  4.869D-03 & -2.844D-04\;\; &  1.540D+01 & -5.064D-01 & -1.728D-04 & -1.133D-04\;\;\cr
 0.301 &  3.847D-01 & -8.315D-03 & -3.109D-03 &  4.496D-05\;\; &  7.963D-01 &  6.922D-01 &  4.727D-03 & -3.554D-04\;\; &  1.017D+01 & -5.250D-01 & -1.888D-04 & -7.917D-05\;\;\cr
 0.401 &  2.354D-01 & -8.443D-03 & -2.945D-03 &  7.496D-05\;\; &  5.297D-01 &  4.401D-01 &  4.537D-03 & -4.483D-04\;\; &  6.642D+00 & -5.094D-01 & -1.921D-04 & -3.139D-05\;\;\cr
 0.501 &  1.356D-01 & -6.803D-03 & -2.745D-03 &  1.078D-04\;\; &  3.511D-01 &  2.759D-01 &  4.299D-03 & -5.575D-04\;\; &  4.369D+00 & -4.710D-01 & -1.559D-04 &  2.607D-05\;\;\cr
 0.601 &  6.999D-02 & -4.005D-03 & -2.517D-03 &  1.399D-04\;\; &  2.314D-01 &  1.696D-01 &  4.026D-03 & -6.759D-04\;\; &  2.905D+00 & -4.214D-01 & -1.329D-04 &  9.206D-05\;\;\cr
 0.701 &  2.753D-02 & -6.161D-04 & -2.271D-03 &  1.677D-04\;\; &  1.509D-01 &  1.010D-01 &  3.723D-03 & -7.969D-04\;\; &  1.954D+00 & -3.686D-01 & -9.700D-05 &  1.655D-04\;\;\cr
 0.801 &  4.582D-04 &  2.934D-03 & -2.014D-03 &  1.878D-04\;\; &  9.615D-02 &  5.674D-02 &  3.401D-03 & -9.133D-04\;\; &  1.330D+00 & -3.179D-01 & -5.520D-05 &  2.439D-04\;\;\cr
 0.901 & -1.602D-02 &  6.331D-03 & -1.755D-03 &  1.975D-04\;\; &  5.867D-02 &  2.803D-02 &  3.068D-03 & -1.018D-03\;\; &  9.156D-01 & -2.720D-01 & -2.272D-06 &  3.232D-04\;\;\cr
 1.001 & -2.542D-02 &  9.380D-03 & -1.503D-03 &  1.946D-04\;\; &  3.276D-02 &  9.419D-03 &  2.735D-03 & -1.105D-03\;\; &  6.341D-01 & -2.314D-01 &  5.797D-05 &  4.029D-04\;\;\cr
 1.101 & -2.979D-02 &  1.191D-02 & -1.264D-03 &  1.783D-04\;\; &  1.502D-02 & -2.510D-03 &  2.410D-03 & -1.171D-03\;\; &  4.398D-01 & -1.962D-01 &  1.235D-04 &  4.774D-04\;\;\cr
 1.201 & -3.084D-02 &  1.384D-02 & -1.043D-03 &  1.485D-04\;\; &  3.259D-03 & -9.659D-03 &  2.100D-03 & -1.213D-03\;\; &  3.051D-01 & -1.657D-01 &  1.914D-04 &  5.447D-04\;\;\cr
 1.301 & -2.998D-02 &  1.518D-02 & -8.456D-04 &  1.066D-04\;\; & -4.328D-03 & -1.347D-02 &  1.812D-03 & -1.229D-03\;\; &  2.110D-01 & -1.393D-01 &  2.594D-04 &  6.032D-04\;\;\cr
 1.401 & -2.780D-02 &  1.591D-02 & -6.730D-04 &  5.441D-05\;\; & -8.879D-03 & -1.509D-02 &  1.550D-03 & -1.220D-03\;\; &  1.457D-01 & -1.169D-01 &  3.250D-04 &  6.477D-04\;\;\cr
 1.501 & -2.479D-02 &  1.610D-02 & -5.266D-04 & -5.290D-06\;\; & -1.119D-02 & -1.529D-02 &  1.317D-03 & -1.189D-03\;\; &  1.004D-01 & -9.791D-02 &  3.850D-04 &  6.793D-04\;\;\cr
 1.601 & -2.191D-02 &  1.591D-02 & -4.047D-04 & -6.941D-05\;\; & -1.229D-02 & -1.462D-02 &  1.114D-03 & -1.136D-03\;\; &  6.860D-02 & -8.194D-02 &  4.353D-04 &  6.964D-04\;\;\cr
 1.701 & -1.899D-02 &  1.538D-02 & -3.066D-04 & -1.348D-04\;\; & -1.255D-02 & -1.351D-02 &  9.400D-04 & -1.068D-03\;\; &  4.652D-02 & -6.873D-02 &  4.755D-04 &  6.988D-04\;\;\cr
 1.801 & -1.622D-02 &  1.457D-02 & -2.300D-04 & -1.984D-04\;\; & -1.219D-02 & -1.215D-02 &  7.941D-04 & -9.879D-04\;\; &  3.138D-02 & -5.790D-02 &  5.046D-04 &  6.879D-04\;\;\cr
 1.901 & -1.371D-02 &  1.360D-02 & -1.723D-04 & -2.574D-04\;\; & -1.149D-02 & -1.070D-02 &  6.739D-04 & -8.993D-04\;\; &  2.088D-02 & -4.894D-02 &  5.229D-04 &  6.649D-04\;\;\cr
 2.001 & -1.154D-02 &  1.254D-02 & -1.296D-04 & -3.099D-04\;\; & -1.066D-02 & -9.310D-03 &  5.756D-04 & -8.059D-04\;\; &  1.375D-02 & -4.175D-02 &  5.296D-04 &  6.320D-04\;\;\cr
 2.101 & -9.675D-03 &  1.141D-02 & -9.989D-05 & -3.541D-04\;\; & -9.740D-03 & -7.972D-03 &  4.970D-04 & -7.120D-04\;\; &  8.848D-03 & -3.585D-02 &  5.265D-04 &  5.907D-04\;\;\cr
 2.201 & -8.117D-03 &  1.028D-02 & -7.934D-05 & -3.892D-04\;\; & -8.886D-03 & -6.797D-03 &  4.337D-04 & -6.199D-04\;\; &  5.557D-03 & -3.123D-02 &  5.139D-04 &  5.441D-04\;\;\cr
 2.301 & -6.862D-03 &  9.182D-03 & -6.584D-05 & -4.148D-04\;\; & -8.079D-03 & -5.735D-03 &  3.834D-04 & -5.318D-04\;\; &  3.260D-03 & -2.744D-02 &  4.938D-04 &  4.942D-04\;\;\cr
 2.401 & -5.746D-03 &  8.061D-03 & -5.774D-05 & -4.311D-04\;\; & -7.264D-03 & -4.790D-03 &  3.437D-04 & -4.494D-04\;\; &  1.817D-03 & -2.447D-02 &  4.681D-04 &  4.419D-04\;\;\cr
 2.501 & -4.754D-03 &  6.925D-03 & -5.210D-05 & -4.390D-04\;\; & -6.440D-03 & -3.932D-03 &  3.107D-04 & -3.733D-04\;\; &  8.937D-04 & -2.206D-02 &  4.370D-04 &  3.912D-04\;\;\cr
 2.601 & -3.896D-03 &  5.777D-03 & -4.913D-05 & -4.392D-04\;\; & -5.633D-03 & -3.152D-03 &  2.847D-04 & -3.060D-04\;\; &  2.644D-04 & -2.001D-02 &  4.041D-04 &  3.410D-04\;\;\cr
 2.701 & -3.160D-03 &  4.668D-03 & -4.683D-05 & -4.331D-04\;\; & -4.874D-03 & -2.440D-03 &  2.629D-04 & -2.460D-04\;\; & -1.439D-04 & -1.823D-02 &  3.694D-04 &  2.940D-04\;\;\cr
 2.801 & -2.499D-03 &  3.589D-03 & -4.483D-05 & -4.211D-04\;\; & -4.160D-03 & -1.814D-03 &  2.444D-04 & -1.929D-04\;\; & -4.162D-04 & -1.662D-02 &  3.338D-04 &  2.501D-04\;\;\cr
 2.901 & -1.957D-03 &  2.602D-03 & -4.285D-05 & -4.056D-04\;\; & -3.538D-03 & -1.287D-03 &  2.281D-04 & -1.482D-04\;\; & -5.767D-04 & -1.522D-02 &  2.996D-04 &  2.102D-04\;\;\cr
 3.001 & -1.456D-03 &  1.665D-03 & -4.031D-05 & -3.870D-04\;\; & -2.955D-03 & -8.248D-04 &  2.132D-04 & -1.097D-04\;\; & -6.466D-04 & -1.393D-02 &  2.660D-04 &  1.753D-04\;\;\cr
 3.101 & -1.087D-03 &  8.782D-04 & -3.741D-05 & -3.671D-04\;\; & -2.502D-03 & -4.903D-04 &  1.995D-04 & -7.772D-05\;\; & -6.775D-04 & -1.282D-02 &  2.346D-04 &  1.433D-04\;\;\cr
 3.201 & -8.082D-04 &  2.024D-04 & -3.415D-05 & -3.459D-04\;\; & -2.130D-03 & -2.430D-04 &  1.872D-04 & -5.123D-05\;\; & -6.945D-04 & -1.179D-02 &  2.051D-04 &  1.163D-04\;\;\cr
 3.301 & -5.949D-04 & -3.586D-04 & -3.030D-05 & -3.245D-04\;\; & -1.841D-03 & -6.112D-05 &  1.748D-04 & -2.929D-05\;\; & -6.672D-04 & -1.095D-02 &  1.781D-04 &  9.261D-05\;\;\cr
 3.401 & -4.416D-04 & -8.563D-04 & -2.668D-05 & -3.036D-04\;\; & -1.615D-03 &  5.790D-05 &  1.635D-04 & -1.184D-05\;\; & -6.497D-04 & -1.019D-02 &  1.541D-04 &  7.254D-05\;\;\cr
 3.501 & -3.380D-04 & -1.229D-03 & -2.288D-05 & -2.838D-04\;\; & -1.446D-03 &  1.078D-04 &  1.529D-04 &  1.821D-06\;\; & -6.073D-04 & -9.538D-03 &  1.323D-04 &  5.553D-05\;\;\cr
 3.601 & -2.548D-04 & -1.590D-03 & -1.884D-05 & -2.653D-04\;\; & -1.305D-03 &  1.403D-04 &  1.426D-04 &  1.276D-05\;\; & -5.735D-04 & -8.950D-03 &  1.127D-04 &  4.119D-05\;\;\cr
 3.701 & -3.003D-04 & -1.760D-03 & -1.476D-05 & -2.474D-04\;\; & -1.289D-03 &  7.839D-05 &  1.324D-04 &  2.140D-05\;\; & -5.790D-04 & -8.425D-03 &  9.546D-05 &  2.966D-05\;\;\cr
 3.801 & -2.796D-04 & -1.976D-03 & -1.119D-05 & -2.318D-04\;\; & -1.231D-03 &  5.794D-05 &  1.235D-04 &  2.756D-05\;\; & -5.466D-04 & -8.003D-03 &  8.061D-05 &  1.973D-05\;\;\cr
 3.901 & -2.138D-04 & -2.269D-03 & -7.747D-06 & -2.179D-04\;\; & -1.131D-03 &  6.653D-05 &  1.146D-04 &  3.219D-05\;\; & -5.126D-04 & -7.516D-03 &  6.789D-05 &  1.093D-05\;\;\cr
 4.001 & -1.926D-04 & -2.433D-03 & -4.371D-06 & -2.045D-04\;\; & -1.045D-03 &  3.904D-05 &  1.063D-04 &  3.530D-05\;\; & -4.771D-04 & -7.074D-03 &  5.643D-05 &  4.836D-06\;\;\cr

